Backprop Diffusion is Biologically Plausible

The Backpropagation algorithm relies on the abstraction of using a neural model that gets rid of the notion of time, since the input is mapped instantaneously to the output. In this paper, we claim that this abstraction of ignoring time, along with the abrupt input changes that occur when feeding the training set, are in fact the reasons why, in some papers, Backprop biological plausibility is regarded as an arguable issue. We show that as soon as a deep feedforward network operates with neurons with time-delayed response, the backprop weight update turns out to be the basic equation of a biologically plausible diffusion process based on forward-backward waves. We also show that such a process very well approximates the gradient for inputs that are not too fast with respect to the depth of the network. These remarks somewhat disclose the diffusion process behind the backprop equation and leads us to interpret the corresponding algorithm as a degeneration of a more general diffusion process that takes place also in neural networks with cyclic connections.

==> constraints0.tex <==
The typical learning paradigm within the framework of NN consists of a
model, that depends on a set of parameters $W$, together with 
an update rule for the parameters; this rule usually is a gradient
descent of a function that measure the goodness
of the model on a specific learning task. However in this section
we will show that when the dynamics of the parameters $W$ is described
by laws that comes from stationarity conditions of a functional, as
it happens for canonical coordinates in classical mechanics (see
Table~\ref{table}), then
the NN model can be treated using the theory of constraints described in the
previous sections. As an immediate  consequence of this approach
the learning process gains temporal and spatial locality even in the
case of recurrent NN.

First of all let us describe the architecture of the models that we will
address. Given a simple digraph $D=(V,A)$ of order $\nu$ without loss of
generality we can assume $V=\{1,2,\dots,\nu\}$ and $A=\{
(i,j)\in\N^2\mid i\in V, j\in V\}$. A neural network constructed on $D$
consists of a set of maps\footnote
{Please notice that now $x$ is a the variable of the variational
problem, and therefore represent a mapping $t\mapsto x(t)$. It not to be
intended as the independent variable of the problem described in the previous sections.} $i\in V\mapsto x^i\in \R$ and $(i,j)\in A\mapsto
w_{ij}\in \R$ together with $\nu$ constraints $G^j(x,W)=0$
$j=1,2,\dots \nu$ where $(W)_{ij}=w_{ij}$. Let ${\cal M}_\nu(\R)$ be the
set of all $\nu\times\nu$ real matrices and 
${\cal M}^{\downarrow}_\nu(\R)$ the set of all $\nu\times\nu$
strictly lower triangular matrices over $\R$. If
$W\in{\cal M}^{\downarrow}_\nu(\R)$ we say that the NN has a feedforward
structure. In this
paper we will consider both feedforward NN and NN with cycles. The relations
$G^j=0$ for $j=1,\dots, \nu$
 specify the computational scheme with which the information
diffuses trough the network. 
In a typical network with $\omega$ inputs these
constraints are defined as follows (see also Fig.~\ref{neuron-const-fig}): 
For any vector $\x\in\R^\nu$, for any matrix $\W\in{\cal
M}_\nu(\R)$ with entries $\w_{ij}$ and for any given ${\cal C}^1$ map 
$e\colon (0,+\infty)\to\R^\omega$ we define the constraint on neuron $j$
when the example $e(\tau)$ is presented to the network as
\begin{equation}G^j(\tau,\x,\W):=\begin{cases}
\x^j-e^j(\tau), & \text{if $1\le j\le \omega$};\\
\x^j-\sigma(\w_{jk} \x^k) & \text{if $\omega <j\le \nu$},
\end{cases}\label{neuron-constraints-structure}\end{equation}
where $\sigma\colon \R\to\R$ is of class ${\cal C}^2(\R)$.

%\begin{figure}
%\[{\vcenter{\|5|}\atop\hbox{(a)}}\qquad\qquad {\vcenter{\|3|}\atop\hbox{(b)}}\]
%\vskip -1pc
%\caption{Visualization of the neural constraints
%for the neural network \protect\<4> (one input $\{1\}$ 
%and two neurons $\{1,2\}$).  Constraint $G^2(x,W)=0$, 
%restricted to the plane $x^1=E^1$, is shown in (a). In (b), 
%such restriction is represented in the  $w_{21}$--$x^2$ plane.}
%\label{neuron-const-fig}
%\end{figure}

Our goal here is to show that such relations , that normally are considered
just a local description of the compositional structure of the NN, once
properly interpreted as constraints in the space $x-W$
%(see Fig.~\ref{neuron-const-fig})
are suitable
holonomic subsidiary conditions in the sense of~\eqref{full-rank-condition}.

Like in the case of classical mechanics, when dealing with learning processes
we are interested in the temporal dynamics of the variables when they are 
exposed to the data from which the learning is supposed to happen. For this
reason in this section we can restrict ourselves to the case $n=1$ and
regard this variable as time  ($x^1=t$). 
Moreover because the neural constraints $G^j(x,W)=0$ involve not only $W$
but also $x$ the $N$ variables $u_1,\dots, u_N$ split into
$x\in \R^\nu$ and $W\in{\cal M}_\nu(\R)$.

\medskip\noindent
{\bf Feedforward Networks.} Now consider the case
$W\in{\cal M}^{\downarrow}_\nu(\R)$
and let us  extend the theory described in Eq.~\eqref{general-functional}
by allowing
$\F(x,W):=\int F(t,x,\dot x,\ddot x,W,\dot W,\ddot W)\, dt$,
so that, in the end, we consider the functional
\begin{equation}
\A(x,W):=\int {1\over 2}(m_x\vert \dot x(t)\vert^2+m_W\vert \dot W(t)\vert^2)\,\varpi(t) dt+
\F(x,W),\label{cognitive-action}\end{equation}
subject to the constraints
\begin{equation}G^j(t,x(t),W(t))=0,\qquad 1\le j\le \nu.
\label{neuron-constraints}\end{equation}
Then the following proposition holds true:
\begin{proposition}
The matrix $({G_\x\atop \overline {G_\W}})\in {\cal M}_{(\nu^2+\nu)\times
\nu}(\R)$ is full rank.
\label{proposition}
\end{proposition}

\begin{proof}
First of all notice that if $(G_\x)_{ij}=G^j_{\x^i}$ is full rank
also $({G_\x\atop \overline {G_\W}})$ has this property. Then, since
\[G^j_{\x^i}(\tau,\x,\W)=\begin{cases}
\delta_{ij}, & \text{if $1\le j\le \omega$};\\
\delta_{ij}-\sigma'(\w_{jk} \x^k)\w_{ji} & \text{if $\omega <j\le \nu$,}
\end{cases}\]
we immediately notice that $G^i_{\x^i}=1$ and that for all $i>j$ we have
$G^i_{\x^i}=0$. This means that
\[
(G^j_{\x^i}(\tau,\x,\W))=\begin{pmatrix}
                          1&*&\cdots&*\\
                          0&1&\cdots&*\\
                          \vdots&\vdots&\ddots&\vdots\\
                          0&0&\cdots&1\end{pmatrix},\]
which is clearly full rank.
\end{proof}
Notice that this result heavily depends on the assumption
$W\in{\cal M}^{\downarrow}_\nu(\R)$; however we will now discuss how
the introduction of an additional variable that models the
degree of satisfaction of the neural constraints acts as a regularizer
of constraints~\eqref{neuron-constraints-structure} and ensure the satisfaction
of~\eqref{full-rank-condition}.

\iffalse
\medskip
\noindent
{\bf Recurrent networks.}
Let us  suppose that
we also assign to each neuron a variable $s$ that measure the degree of
violation of the constraint. Then Eq.~\eqref{neuron-constraints} assumes
the form $G^j(t,x,W,s)=0$, $j=1,2,\dots,\nu$ where
\begin{equation}
G^j(\tau,\x,\W,\s):=\begin{cases}
\x^j-e^j(\tau)+\s^j, & \text{if $1\le j\le \omega$;}\\
\x^j-\sigma(\w_{jk} \x^k)+\s^j & \text{if $\omega <j\le \nu$}.
\end{cases}\label{neuron-constraints-slack}\end{equation}
In doing so it is important to notice that Proposition~\ref{proposition} holds
without the assumption that $\W\in{\cal M}^\downarrow_\nu(\R)$ as it is
immediate to prove since $G^j_{\s^i}=\delta_{ij}$,
which is of course full rank. This important remark opens the possibility to
extend the theory to  networks with ``feedback'' connections
based on general simple digraphs.

In this formulation of the theory the action, described in Eq.~\eqref{cognitive-action} must be modified to take into account of the introduction of
the new variable $s$:
\begin{equation}
\A(x,W,s):=\int {1\over 2}(m_x\vert \dot x(t)\vert^2+m_W\vert \dot W(t)\vert^2
+m_s\vert \dot s(t)\vert^2)\,\varpi(t) dt
+\F(x,W,s),\label{cognitive-action-slack}
\end{equation}
where $\F(x,W,s):=\int F(t,x,\dot x,\ddot x,W,\dot W,\ddot W,s)\, dt$.
\fi
% Local Variables:  
% mode: latex
% TeX-master: "neurips_2019-ccal.tex"
% End:

==> dirichlet.tex <==
Let $\Omega$ be an open, bounded domain in $\R^n$, let
$u\colon\Omega\to \R^N$, $\varpi\in{\cal
C}^1(\Omega; (0,+\infty))$ and $\F(u):= \int_\Omega F(x,u,\nabla u)\,dx$ be, and
define the following functional
\begin{equation}
\S(u):=\frac{1}{2}\int_\Omega \vert\nabla u(x)\vert^2\, \varpi(x)dx+\F(u),
\label{general-functional}\end{equation}
which is a weighted Dirichlet integral plus the $\F(u)$ term. We are here
interested in the necessary conditions for $u$ to be an extremizer of the
{\it modified Dirichlet functional} \eqref{general-functional} subject to
a class of  holonomic constraints of the form
\footnote{In this section, for the sake of simplicity, we are considering
holonomic constraints that do not depend explicitly on the independent
variable $x$, however the arguments presented here can be readily generalized
also to include the case $G(x,u(x))=0$. Indeed in
Section~\ref{constraint-sec} we will consider general holonomic constraints.
} $G(u(x))=0$. Let us consider the problem in Eq.~\eqref{general-functional} where
$u$ is subject to the constraints $G(u(x))=0$ for all $x\in \overline\Omega$
and $G(z)$ of class ${\cal C}^2(\R^N, \R^r)$. Furthermore assume that
the $r\times N$ Jacobian  matrix defined by  $G_z=(G^i_{z^j})$
satisfies\footnote{We could ask for a less restrictive condition here, namely that
$G_z(z)$ should be full rank on all the points $z\in\R^N$ such that
$G(z)=0$.}:
\begin{equation}
\rank G_z=r\quad\hbox{for
all  $z\in \R^N$}.
\label{full-rank-condition}
\end{equation}
From the theory of calculus of variation with subsidiary conditions
(see \cite{giaquita-hildebrandt} Chap.~2) we know that there exist
$\lambda_1,\dots,\lambda_r\in {\cal C}^0(\Omega)$ such that the
constrained stationary points of $\S$ coincides with the unconstrained
stationary points of the extended functional
\begin{equation}
\S^*(u)={1\over 2}\int_\Omega \vert \nabla u(x)\vert^2\varpi(x)-
\lambda_j(x)G^j(u(x))\, dx+\F(u),
\label{const-func-gen}\end{equation}
and the Euler equation for this functional are
\footnote{throughout this paper we will adopt Einstein summation convention;
that is to say two repeated indices,
unless otherwise specified imply summation.}
\begin{equation}
-\varpi\Delta u -u_{x^\alpha}\varpi_{x^\alpha}-\lambda_\ell G^\ell_z(u)
+L_F(u)=0,\label{ELE-gen-mult}\end{equation}
where $L_F(u)$ is the Euler operator (\cite{giaquita-hildebrandt} p. 18 and
\cite{courant-hilbert}).
Differentiating the constraints two times with respect to
$x^\alpha$ one obtaines
\begin{equation}
-\Delta u\cdot G_z^j(u)=G^j_{z^iz^k}(u)u^i_{x^\alpha}u^k_{x^\alpha},
\qquad 1\le j\le r.
\end{equation}
Hence if we scalar  multiply Euler equation by $G_z^j(u)$ we obtain
\begin{equation}A_{ij}(u)\lambda_\ell=\varpi
G^j_{z^iz^k}(u)u^i_{x^\alpha}u^k_{x^\alpha}-\varpi_{x^\alpha}(u_{x^\alpha}\cdot
G^j_z(u)) +L_F(u)\cdot G_z^j(u),
\label{mult-lin-eq}
\end{equation}
where we defined  $A_{j\ell}(u):=G_z^j(u)\cdot G^\ell_z(u)$.
Therefore  Euler equations for the constrained
functional~\eqref{const-func-gen}  are~\eqref{ELE-gen-mult}
with
\begin{equation}
\lambda_\ell=(A^{-1}(u))_{\ell j}\bigl(\varpi
G^j_{z^iz^k}(u)u^i_{x^\alpha}u^k_{x^\alpha}
-\varpi_{x^\alpha}(u_{x^\alpha}\cdot G^j_z(u))
+L_F(u)G_z^j(u)\bigr).
\label{mult-eq-gen}
\end{equation}
Notice that in order to get from Eq.~\eqref{mult-lin-eq} to
\eqref{mult-eq-gen} we need to know that
$A$ is invertible. Whenever our assumption~\eqref{full-rank-condition} holds
the Gram matrix $A(u)$ turns out to be a invertible in view of the following
(well known) lemma:

\begin{lemma}
If $v_1$,\dots, $v_n$ are $n$ linear independent vectors, then the Gram matrix
$G_{ij}:=(v_i,v_j)$ is positive definite.
\end{lemma}

\begin{proof}
$(x,Gx)=x_i(v_i,v_j)x_j=(x_i v_i, x_j v_j)=\Vert v_i x_i\Vert^2\ge 0$.
However $\Vert v_i x_i\Vert=0$ if and only if $x_iv_i=0$, therefore
we can conclude that $(x,Gx)>0$ for every $x\ne 0$.
\end{proof}




% Local Variables:  
% mode: latex
% TeX-master: "neurips_2019-ccal.tex"
% End:

==> dirichlet0.tex <==
In the remainder of the paper we show that the forward/backward
diffusion of layered networks is just a special case of more
general diffusion processes that are at the basis of learning
in neural networks characterized by graphs with any pattern of
interconnections. In particular we show that 
this naturally arises when formulating 
learning as a parsimonious constraint satisfaction problem.
We begin presenting a general result which makes it possible 
to determine the Lagrangian multipliers in variational problems
with subsidiary conditions~\cite{Giaquinta1996-1}. 
%qui

Let $\Omega$ be an open, bounded domain in $\R^n$, let
$u\colon\Omega\to \R^N$, $\varpi\in{\cal
C}^1(\Omega; (0,+\infty))$ and $\F(u):= \int_\Omega F(x,u,\nabla u)\,dx$, and
define the following functional
\begin{equation}
\S(u):=\frac{1}{2}\int_\Omega \vert\nabla u(x)\vert^2\, \varpi(x)dx+\F(u),
\label{general-functional}\end{equation}
which is a weighted Dirichlet integral plus the $\F(u)$ term. We are here
interested in the necessary conditions for $u$ to be an extremizer of the
{\it modified Dirichlet functional} \eqref{general-functional} subject to
a class of  holonomic constraints of the form
%\footnote{In this section, for the sake of simplicity, we are considering
%holonomic constraints that do not depend explicitly on the independent
%variable $x$, however the arguments presented here can be readily generalized
%also to include the case $G(x,u(x))=0$. Indeed in
%Section~\ref{constraint-sec} we will consider general holonomic constraints.
%} $G(u(x))=0$.

Consider the problem in Eq.~\eqref{general-functional} where
$u$ is subject to the constraints $G(u(x))=0$ for all $x\in \overline\Omega$
and $G(z)$ of class ${\cal C}^2(\R^N, \R^r)$. Furthermore assume that
the $r\times N$ Jacobian  matrix defined by  $G_z=(G^i_{z^j})$
satisfies\footnote{We could ask for a less restrictive condition here, namely that
$G_z(z)$ should be full rank on all the points $z\in\R^N$ such that
$G(z)=0$.}:
\begin{equation}
\rank G_z=r\quad\hbox{for
all  $z\in \R^N$}.
\label{full-rank-condition}
\end{equation}
From the theory of calculus of variation with subsidiary conditions
(see \cite{giaquita-hildebrandt} Chap.~2) we know that there exist
$\lambda_1,\dots,\lambda_r\in {\cal C}^0(\Omega)$ such that the
constrained stationary points of $\S$ coincides with the unconstrained
stationary points of the extended functional
\begin{equation}
\S^*(u)={1\over 2}\int_\Omega \vert \nabla u(x)\vert^2\varpi(x)-
\lambda_j(x)G^j(u(x))\, dx+\F(u),
\label{const-func-gen}\end{equation}
and the Euler equation for this functional are
\footnote{throughout this paper we will adopt Einstein summation convention;
that is to say two repeated indices,
unless otherwise specified imply summation.}
\begin{equation}
-\varpi\Delta u -u_{x^\alpha}\varpi_{x^\alpha}-\lambda_\ell G^\ell_z(u)
+L_F(u)=0,\label{ELE-gen-mult}\end{equation}
where $L_F(u)$ is the Euler operator (\cite{giaquita-hildebrandt} p. 18 and
\cite{courant-hilbert}).
Differentiating the constraints two times with respect to
$x^\alpha$ one obtaines
\begin{equation}
-\Delta u\cdot G_z^j(u)=G^j_{z^iz^k}(u)u^i_{x^\alpha}u^k_{x^\alpha},
\qquad 1\le j\le r.
\end{equation}
Hence if we scalar  multiply Euler equation by $G_z^j(u)$ we obtain
\begin{equation}A_{ij}(u)\lambda_\ell=\varpi
G^j_{z^iz^k}(u)u^i_{x^\alpha}u^k_{x^\alpha}-\varpi_{x^\alpha}(u_{x^\alpha}\cdot
G^j_z(u)) +L_F(u)\cdot G_z^j(u),
\label{mult-lin-eq}
\end{equation}
where we defined  $A_{j\ell}(u):=G_z^j(u)\cdot G^\ell_z(u)$.
Therefore  Euler equations for the constrained
functional~\eqref{const-func-gen}  are~\eqref{ELE-gen-mult}
with
\begin{equation}
\lambda_\ell=(A^{-1}(u))_{\ell j}\bigl(\varpi
G^j_{z^iz^k}(u)u^i_{x^\alpha}u^k_{x^\alpha}
-\varpi_{x^\alpha}(u_{x^\alpha}\cdot G^j_z(u))
+L_F(u)G_z^j(u)\bigr).
\label{mult-eq-gen}
\end{equation}
Notice that in order to get from Eq.~\eqref{mult-lin-eq} to
\eqref{mult-eq-gen} we need to know that
$A$ is invertible. Whenever our assumption~\eqref{full-rank-condition} holds
the Gram matrix $A(u)$ turns out to be a invertible in view of the following
(well known) lemma:

\begin{lemma}
If $v_1$,\dots, $v_n$ are $n$ linear independent vectors, then the Ghram matrix
$G_{ij}:=(v_i,v_j)$ is positive definite.
\end{lemma}

\begin{proof}
$(x,Gx)=x_i(v_i,v_j)x_j=(x_i v_i, x_j v_j)=\Vert v_i x_i\Vert^2\ge 0$.
However $\Vert v_i x_i\Vert=0$ if and only if $x_iv_i=0$, therefore
we can conclude that $(x,Gx)>0$ for every $x\ne 0$.
\end{proof}


\begin{table}
\small
\begin{tabular}{ccl}  
\toprule
{\bf Learning}  & {\bf Mechanics} & {\bf Remarks} \\
\midrule
$(W,x)$       & $u$  & 
                       Weights and neuronal outputs
                       are interpreted as generalized
                       coordinates.\\
\noalign{\smallskip}
$(\dot W,\dot x)$& $\dot u$ & 
                              Weight variations and neuronal variations
                              are interpreted as generalized velocities.
                              \\
\noalign{\medskip}
  $\A(x,W)$ & $\S(u)$&  
                       The cognitive action is the dual of the action in
                       mechanics.
                       \\
\bottomrule
\end{tabular}
\medskip
\caption{Links between learning theory and classical mechanics.}
\label{table}
\end{table}

% Local Variables:  
% mode: latex
% TeX-master: "neurips_2019-ccal.tex"
% End:

==> laws0.tex <==
Now we concentrated ourselves on showing that the set of
constraints that define a NN are good constraints (in the sense
of~\eqref{full-rank-condition}). In this section we  will focus on the
feedforward case described by the functional~\eqref{cognitive-action}
together with constraints~\eqref{neuron-constraints}. In particular we
will discuss the updates rules (Euler equations) for the variables $x$ and
$W$ derived from the stationarity conditions of the
functional~\eqref{cognitive-action}.

% We now turn to the problem of showing
% what are the update rules for the Lagrangian variables $x$, $W$ and $s$
% prescribed by the stationarity conditions of the functional $\A$.
% All the results will be derived assuming the general form of $\A$
% defined in~\eqref{cognitive-action} and \eqref{cognitive-action-slack}.
% It is clear that only special forms of $F$ are suitable for learning tasks.
% At the end of this section  we will, just for the case of feedforward NN,
% show how these differential rules that we find
%  are intimately related
% to the usual gradient dynamics of the weights that is considered
% in machine learning. In fact we will argue that this approach
% represent a generalization of standard gradient methods.


We begin by deriving
the constrained Euler equations associated with the
functional~\eqref{cognitive-action} under
subsidiary conditions~\eqref{neuron-constraints}. The
constrained functional is
\begin{equation}
\A\ ^*(X,W)=\int {1\over 2}(m_x\vert \dot x(t)\vert^2+m_W\vert \dot W(t)\vert^2)\varpi(t)
-\lambda_j(t)G^j(t,x(t),W(t))\, dt+\F(x,W),
\end{equation}
and its Euler equations thus read

\begin{align}
  &-m_x\varpi(t)\ddot x(t)-m_x\dot\varpi(t) \dot x(t)
  -\lambda_j(t)G^j_\x(x(t),W(t))
+L^x_F(x(t),W(t))=0;\label{x-eq}\\
  &-m_W\varpi(t)\ddot W(t)-m_W\dot\varpi(t) \dot W(t)
  -\lambda_j(t)G^j_\W(x(t),W(t))
+L^W_F(x(t),W(t))=0,\label{W-eq}
\end{align}
where $L_F^x=F_x-d(F_{\dot x})/dt+d^2(F_{\ddot x})/dt^2$,
$L_F^W=F_W-d(F_{\dot W})/dt+d^2(F_{\ddot W})/dt^2$
are the functional derivatives of $F$ with respect to $x$ and $W$
respectively (see \cite{courant-hilbert}). An expression for Lagrange
multiplies, as it is explained in Section~\ref{dirichlet-sec}
is derived by differentiating two times the constraint with respect to the
time and using the obtained expression to substitute the second order terms
in the Euler equations. In this case the analogue of Eq.~\eqref{mult-lin-eq}
is
\begin{equation}
\begin{aligned}
\Bigl({G^i_{\xi^a}G^j_{\xi^a}\over m_x}+{G^i_{m_{ab}}G^j_{m_{ab}}
\over m_W}\Bigr)\lambda_j=&
\varpi\bigl(G^i_{\tvar\tvar}+2(G^i_{\tvar \x^a}\dot x^a
+G^i_{\tvar \w_{ab}}\dot w_{ab}
+G^i_{\x^a\w_{bc}}\dot x^a\dot w_{bc})\\
&+G^i_{\x^a\x^b}\dot x^a \dot x^b
+G^i_{\w_{ab}\w_{cd}}\dot w_{ab}\dot w_{cd}\bigr)\\
&-\dot \varpi( \dot x^a G^i_{\xi^a}+\dot w_{ab} G^i_{m_{ab}})
+{L^{x^a}_FG^i_{\xi^a}\over m_x}+{L^{w_{ab}}_FG^i_{m_{ab}}\over m_W},
\end{aligned}\label{mult-lin-eq-x-w}
\end{equation}
where $G^i_\tvar$, $G^i_{\tvar\tvar}$, $G^i_{\xi^a}$, $G^i_{\xi^a\xi^b}$,
$G^i_{\w_{ab}}$ and  $G^i_{\w_{ab}\w_{cd}}$ are the gradients and the
hessians of constraint~\eqref{neuron-constraints}.

% The components of the gradient and of the hessian of $G$
% are (with no sum over $j$):
% \begin{equation}
% G^j_{\x^a}(\x,\W)=\begin{cases}
% \delta_{aj}, & \text{if $1\le j\le \omega$;}\\
% \delta_{aj}-\sigma'(\w_{jk} \x^k)\w_{ja} & \text{if $\omega <j\le \nu$,}
% \end{cases}\label{G_xi}\end{equation}
% \begin{equation}
% G^j_{\x^a\xi^b}(\x,\W)=\begin{cases}
% 0, & \text{if $1\le j\le \omega$;}\\
% -\sigma''(\w_{jk} \x^k)\w_{ja} \w_{jb} & \text{if $\omega <j\le \nu$,}
% \end{cases}\end{equation}
% \begin{equation}G^j_{\w_{ab}}(\x,\W)=\begin{cases}
% 0, & \text{if $1\le j\le \omega$;}\\
% -\sigma'(\w_{jk} \x^k)\x^b\delta_{aj} & \text{if $\omega <j\le \nu$,}
% \end{cases}\end{equation}
% \begin{equation}G^j_{\w_{ab}\w_{cd}}(\x,\W)=\begin{cases}
% 0, & \text{if $1\le j\le \omega$;}\\
% -\sigma''(\w_{jk} \x^k)\x^b\x^d\delta_{aj}\delta_{cj} & \text{if $\omega <j\le \nu$,}
% \end{cases}\end{equation}
% \begin{equation}G^j_{\x^a\w_{bc}}(\x,\W)=\begin{cases}
% 0, & \text{if $1\le j\le \omega$;}\\
% \begin{aligned}&-\bigl(\sigma'(\w_{jk} \x^k)\delta_{ac}\\&+\sigma''(\w_{jk} \x^k)
% \x^c\w_{ja}\bigr)\delta_{jb}\end{aligned}& \text{if $\omega <j\le \nu$.}\label{G_xim}
% \end{cases}
% \end{equation}
% All the remaining terms in Eq.~\eqref{x-eq}, \eqref{W-eq} and \eqref{multiplier}
% depend on the specific form of
% $F$.
% For example if we consider the case of supervised learning, 
% since the loss function typically depends only on the value of the output
% neurons and on the supervisions, we will have $L_F^W\equiv 0$.

% with $\outputs$ outputs the term $F$ can be chosen as 
% $F(t,x,\dot x,\ddot x,W,\dot W,\ddot W)=
% -\varpi(t)/2\sum_{i=1}^\outputs(y^i(t)-x^{\nu-\outputs+i}(t))^2$,
% where $y\in\R^\outputs$ is a supervision signal. In this specific case
% we have $L_F^W\equiv 0$.

\medskip
\noindent
{\bf Initial conditions. }
Suppose now that we want to solve Eq.~ \eqref{x-eq}--\eqref{W-eq}
with Cauchy initial conditions.
Of course we must choose $W(0)$ and $x(0)$ such that $g_i(0)\equiv 0$, where
we posed $g_i(t):= G^i(t, x(t), W(t))$, for $i=1,\dots,\nu$. However since the
constraint must hold also for all $t\ge0$ we must also have at least
$g'_i(0)=0$. These conditions written explicitly means
\[G^i_\tau(0,x(0),W(0))+G^i_{\xi^a}(0,x(0),W(0))\dot x^a(0)
+G^i_{m_{ab}}(0,x(0),W(0))\dot w_{ab}(0)=0.\]
If the constraints does not depend explicitly on time it is sufficient to
to choose $\dot x(0)=0$ and $\dot W(0)=0$, while for time dependent constraint
this condition leaves 
\[G^i_\tau(0,x(0),W(0))=0,\]
which is an additional constraint on the initial conditions $x(0)$ and $W(0)$
to be satisfied.
Therefore one possible consistent way to impose Cauchy conditions
\begin{equation}
\begin{aligned}
&G^i(0,x(0),W(0))=0,\quad i=1,\dots,\nu;\\
&G^i_\tau(0,x(0),W(0))=0,\quad i=1,\dots,\nu;\\
&\dot x(0)=0;\\
&\dot W(0)=0.
\end{aligned}
\label{initial-cond}
\end{equation}
Higher derivative of $g_i(0)$ becomes automatically satisfied thanks
through the differential equations.

% \medskip
% \noindent
% {\bf Recurrent case.}
% In this case the Euler equations associated with the
% problem~\eqref{cognitive-action-slack} under the conditions $G^j(x,W,s)=0$
% are
% \begin{align}
% &\begin{aligned}\varpi(t) \ddot x(t)+\dot\varpi(t) \dot x(t)
% &+\lambda_j(t)G^j_\x(x(t),W(t),s(t))\\
% &-L^x_F(x(t),W(t),s(t))=0;
% \end{aligned}\label{x-eq-slack}\\
% &\begin{aligned}\varpi(t) \ddot W(t)+\dot\varpi(t) \dot W(t)
% &+\lambda_j(t)G^j_\W(x(t),W(t),s(t))\\
% &-L^W_F(x(t),W(t),s(t))=0,
% \end{aligned}\label{W-eq-slack}\\
% &\begin{aligned}
% \varpi(t) \ddot s(t)+\dot\varpi(t) \dot s(t)
% &+\lambda_j(t)G^j_\s(x(t),W(t),s(t))\\
% &-L^s_F(x(t),W(t),s(t))=0,\cr
% \end{aligned}\label{s-eq-slack}
% \end{align}
% where $L^\s_F=F_\s$.
% Notice that in the above expressions the new variable $s$
% will appear also in the lagrange multipliers.
% Here
% \begin{equation}
% \begin{aligned}
% \lambda_\ell=A^{-1}_{\ell j}\Bigl(&\varpi G^j_{\x^a\x^b}\dot x^a\dot x^b
% +\varpi G^j_{\w_{ab} \w_{cd}}\dot W_{ab} \dot W_{cd}\\
% &+\varpi G^j_{\x^a \w_{bc}}\dot x^a\dot W_{bc}
% -\dot\varpi (\dot x^a G^j_{\x^a}+\dot W_{ab} G^j_{\w_{ab}}+\dot s^j)\\
% &+L_F^x\cdot G^j_\x+L_F^W\cdot G^j_\W+F_{\s^j}\Bigr),
% \end{aligned}
% \end{equation}
% with $A_{ij}=\delta_{ij}+G^i_{\x^a} G^j_{\x^a}+G^i_{\w_{ab}} G^j_{\w_{ab}}$,
% while Eq.~\eqref{G_xi}--\eqref{G_xim} remains unchanged.

\medskip
\noindent
{\bf Supervised Learning and reduction to BP.}
In order to see how this theory can be readily
applied to learning let us restrict ourselves to the case
$W\in {\cal M}^\downarrow_\nu(\R)$ and choose $\varpi(t)=\exp(\vartheta t)$,
$\vartheta>0$, $m>0$.
Now let us choose
\[F(t,x(t),\dot x(t), \ddot x(t),W(t),\dot W(t),\ddot W(t))=-e^{\vartheta t}
V(x(t),y(t)),\]
where $y(t)$ is an assigned supervision signal and
\[V(x(t),y(t)):=\frac{1}{2}\sum_{i=1}^\outputs
(y^i(t)-x^{\nu-\outputs+i}(t))^2,\]
$x^{\nu-\outputs},\dots, x^{\nu}$ being the variables associated with
the outputs neurons. A typical input signal and the corresponding
supervision signal can be constructed from
a standard training set $\mathscr{L}:=\{(e_\kappa, d_\kappa)
\mid e_\kappa \in \R^\omega, d_\kappa\in\R^\eta, \kappa=1,\dots,\ell \}$
in the following manner. Choose a sequence of times $\langle t_n\rangle:=t_0,t_1,t_2,\dots$
such that $|t_{i+1}-t_i|=:\tau$ is constant $i\in\N$. Furthermore
define the following sequences: $\langle E_n\rangle:=
e_1,\dots, e_\ell,e_1,\dots e_\ell,\dots$ and
$\langle y_n\rangle:= d_1,\dots, d_\ell,d_1,\dots d_\ell,\dots$.
Let $R(t):= \sum_{n=0}^\infty \rho_\epsilon(t-t_n)$, where
$\rho_\epsilon(\cdot)$ are standard Friedrichs mollifiers and define
\[\bar E(t):=\sum_{n=0}^\infty E_n \chi_{[t_{n-1},t_n]}(t),\quad
\bar y(t):=\sum_{n=0}^\infty y_n \chi_{[t_{n-1},t_n]}(t),\]
where $\chi_A$ is the characteristic function of the set $A$ and
$t_{-1}=0$.
Then the signal
\[E(t):=(\bar E *R)(t),\quad{\rm and}\quad y(t):=(\bar y *R)(t),\]
is piecewise constant signals with smooth transitions. 

\iffalse
The temporal
behaviour of these signals is depicted in the side figure.
%
% \begin{figure}[t]
% \begin{center}
% \[\]
% \caption{Temporal behavior of the input and  supervision signal.}
% \label{signals-figs}
% \end{center}
% \end

\smash{\raise-2pc\rlap{\kern23pc\vbox{
\hbox{\includegraphics{./figs/qpe-3.mps}}}}}
\parshape 3 0pt 22pc 0pt 22pc 0pt \hsize
\fi
In order to understand the behaviour of the Euler equations~\eqref{x-eq}
and~\eqref{W-eq} 
we observe that in the case of feedforward networks, as it
is well known, the constraints
$G^j(t,x,W)=0$ can be solved for $x$ so that eventually we can express the
value of the output neurons in terms of the value of the input neurons.
If we let $f^i_W(e(t))$ be the value of $x^{\nu-i}$ when $x^1=e^1(t),\dots
,x^\omega=e^\omega(t)$, then the theory defined by \eqref{cognitive-action} under
subsidiary conditions~\eqref{neuron-constraints} is equivalent, when
$m_x=0$, to the 
unconstrained theory defined by
\begin{equation}
\int e^{\vartheta t}\Bigl(\frac{m_W}{2}\vert\dot W\vert^2-\overline V(t,W(t))
\Bigr)\, dt\label{supervised-unconstrained}
\end{equation}
where $\overline V(t,W(t)):=\frac{1}{2}\sum_{i=1}^\outputs
(y^i(t)-f^i_W(E(t)))^2$. The Euler equations associated
with~\eqref{supervised-unconstrained} are
\begin{equation}
\ddot W(t)+\vartheta \dot W(t)=-\frac{1}{m_W}\overline V_W(t,W(t)),
\label{euler-backprop}
\end{equation}
that in the limit $\vartheta\to\infty$ and $\vartheta m\to \gamma$ reduces to
the gradient method
\begin{equation}
\dot W(t)=-\frac1\gamma \overline V_W(t,W(t)),
\label{gradient-like-w}
\end{equation}
with learning rate $1/\gamma$.
Notice that the presence of the term $\varpi(t)$ that we proposed in the
general theory it is essential in order
to have a learning behaviour as it produce dissipation.

Typically the term $\overline V_W(t,W(t))$ in Eq.~\eqref{gradient-like-w}
can be evaluated using the Backpropagation algorithm; we will now show that
Eq.~\eqref{x-eq}--\eqref{mult-lin-eq-x-w} in the same limit used above
$m_x\to 0$, $m_W\to 0$, $m_x/m_W\to 0$ reproduces Eq.~\eqref{gradient-like-w}
where the term $\overline V_W(t,W(t))$ explicitly assumes the form
prescribed by BP. In order to see this choose $\vartheta=\gamma/m_W$ and
multiply both sides of Eq.~\eqref{x-eq}--\eqref{mult-lin-eq-x-w} by
$\exp(-\vartheta t)$, then take the limit
$m_x\to 0$, $m_W\to 0$, $m_x/m_W\to 0$. In this limit Eq.~\eqref{W-eq} and
Eq.~\eqref{mult-lin-eq-x-w} becomes respectively
\begin{align}
&\dot W=-\frac1\gamma  \sigma'(w_{ik}x^k) \delta_i x^j;\label{BP-grad}\\
&G^i_{\xi^a} G^j_{\xi^a} \delta_j=-V_{x^a}G^i_{\xi^a},\label{backward}
\end{align}
where $\delta_j$ is the limit of $\exp(-\vartheta t)\lambda_j$.
Because the matrix $G^i_{\x^a}G^j_{\x^a}$ not only is invertible,
but it is a Gram matrix if we define $T_{ij}:= G^j_{\xi^i}$, then
we have $G^i_{\x^a}G^j_{\x^a}=(T'T)_{ij}$. If we then  pose
$v_i:=-\gamma G^i_{\x^a}\dot x^a$, the $\delta$'s  satisfies
$T'T\delta=v$ with $T$ that is an upper triangular matrix. Solving this
equation is equivalent to the solution of $T'\mu= v$ and $T\delta=\mu$.
From this last equation we immediately see that once $\mu$ is known
the $\delta$ are recursively derived starting from the output neurons.
Once we understood this it becomes apparent that if we identify $\delta_i$
with the BP delta-error Eq.~\eqref{backward} is the recursive relation
of the delta-errors while Eq.~\eqref{BP-grad} is a gradient descent method
with the gradient evaluated with the BP rule.


% The same limit process applied
% to  Eq.~\eqref{x-eq} and~\eqref{W-eq} gives equations with the following form: 
% \begin{align}
%   &\dot x(t)
%   +C^\gamma_j(t)G^j_\x(x(t),W(t))
% =-\frac{1}{\gamma}V_x(x(t), y(t));\label{x-eq}\\
%   &\dot W(t)
%   +C^\gamma_j(t)G^j_\W(x(t),W(t))=0,\label{W-eq}
% \end{align}
% where $C_j^\gamma$ is the limit value of $\lambda_j$ as
% $\vartheta\to0$ and $\vartheta m\to 1/\gamma$, thus showing us clearly that
% ${\dot x\choose \dot W}$ lies in the linear span of the
% normal vectors to the constraints active at the point
% ${x\choose W}$ and the vector ${V_x\choose0}$.

% Equation~\eqref{euler-backprop} is extremely useful in order to understand
% what the dynamic of Eq.~\eqref{x-eq} and~\eqref{W-eq} looks like, since
% they comes form equivalent problems. However there is a crucial difference
% between the two formulations that is the whole point of the paper: In order to
% evaluate the term $\overline V_W(t,W(t))$ in Eq.~\eqref{euler-backprop}
% non-local calculations in space are required; on the other hand
% Eq.~\eqref{x-eq} and~\eqref{W-eq} and also Eq.~\eqref{x-eq-slack},
% \eqref{W-eq-slack} and~\eqref{s-eq-slack} are manifestly local both in time
% and in space.

\iffalse
\subsection{Simulation of the dynamic}
In order to prove the soundness of the proposed theory we performed
some simulations of the Euler equations Eq.~\eqref{x-eq} and~\eqref{W-eq}
in the special case $\omega=1$, $\eta=1$, $\varpi=\exp(\vartheta t)$ and
$F=-\exp(\vartheta t) \overline V(t,x(t))$, where in particular
$\overline V(t,x(t))$ is taken to be a quadratic loss on the output neuron.


In order to understand the learning dynamic of the weight
we choose a constant supervision signal and various input signals $e(t)$.
Figure~\ref{experim1} shows the evolution of the weight of a single 
linear neuron $x(t)=w(t) e(t)$
with a target $y=3$ and a variable input $e(t)$. In
Fig.~\ref{experim1}--(a) $e(t)\to 3$ as $t\to\infty$, and indeed
$w(t)$ converges to $1$. In
Fig.~\ref{experim1}--(b) $e(t)\approx 3(1-t)$ and consistently $w(t)\approx
1/(1-t)$. Notice that in both cases the neuron constraint is always satisfied.
Remember that the initial conditions must be consistent with
Eq.~\eqref{initial-cond}; in this example indeed in Fig.~\ref{experim1}--(a)
we have $w(0)=0$ that guaranteed $G_\tau=0$, while in the experiment
relative to Fig.~\ref{experim1}--(b) one can choose $\dot w(0)\ne 0$ as
$G_\tau=0$ is ensured by $\dot e(0)=0$.

In Fig.~\ref{experim2} instead  we tested the robustness of the method
with respect to numerical errors by running the simulation for a longer
period of time. The model here consists of  two neurons NN with nonlinear
activation function. We observed that due to numerical errors the system
can fail to converge to the correct solution $w=1$
(Fig.~\ref{experim2}--(a)). This can be understood as soon as we realize that,
following the ideas of Section~\ref{dirichlet-sec}, Euler equations
implements only the satisfaction of the second derivative of the
constraints, therefore small errors on the trajectories can shift the dynamic
of the system on another constraint that differs from the correct one by
a linear function of time.
Because of this we found that such behaviour can be effectively
corrected (see Fig.~\ref{experim2}--(b))
by adding an additional term on the potential a quadratic loss
on the constraint itself.

%\def+#1+{\vbox{\includegraphics[width=0.5\hsize]{figs/#1}}}
 \begin{figure}[t]
 %\<<ex0-lin-var-w0_0.pdf>>
\hbox to\hsize{
\includegraphics[width=0.5\hsize]{figs/ex0-1.eps}\hfill
\includegraphics[width=0.5\hsize]{figs/ex0-2.eps}
}
\hbox to \hsize{\hfil(a)\qquad\quad\hfil\quad\qquad(b)\hfil}
\caption{Temporal evolution for the weights of a linear neuron
characterized by the constraint $G=x(t)-w(t)e(t)$. We used
$\overline V=(x-3)^2/2$ and we fixed the parameters as follows
$m_x=m_W=\vartheta=1$. The shown trajectories correspond to
the initial conditions $\dot w(0)=\dot x(0)=x(0)=0$, $w(0)=0$ in
(a), and $w(0)=0.01$ in (b).}
\label{experim1}
\end{figure}
\begin{figure}
\hbox to\hsize{
\includegraphics[width=0.5\hsize]{figs/ex1-not-augmented.eps}\hfill
\includegraphics[width=0.5\hsize]{figs/ex1-augmented.eps}
}
\hbox to \hsize{\hfil(a)\qquad\quad\hfil\quad\qquad(b)\hfil}
\caption{Temporal evolution of the weight that connects two neurons:
$G^1=x^1-e$, $G^2=x^2-\sigma(w x^1)$ with $\sigma(x):=\Th(x)$. We took
$m_x=m_W=\vartheta=1$ and identically null initial conditions.
In (a) we considered $\overline V=(x^2-\Th(3))^2/2$, while in (b)
we chose $\overline V=(x^2-\Th(3))^2/2+(x^2-\sigma(w x^1))^2/2$. 
}
\label{experim2}
\end{figure}
\fi
% Local Variables:  
% mode: latex
% TeX-master: "neurips_2019-ccal.tex"
% End:
